Low-latency D-MIMO Localization using Distributed Scalable Message-Passing Algorithm

Distributed MIMO and integrated sensing and communication are expected to be key technologies in future wireless systems, enabling reliable, low-latency communication and accurate localization. Dedicated localization solutions must support distributed architecture, provide scalability across different system configurations and meet strict latency requirements. We present a scalable message-passing localization method and architecture co-designed for a panel-based distributed MIMO system and network topology, in which interconnected units operate without centralized processing. This method jointly detects line-of-sight paths to distributed units from multipath measurements in dynamic scenarios, localizes the agent, and achieves very low latency. Additionally, we introduce a cycle-accurate system latency model based on implemented FPGA operations, and show important insights into processing latency and hardware utilization and system-level trade-offs. We compare our method to a multipath-based localization method and show that it can achieve similar localization performance, with wide enough distribution of array elements, while offering lower latency and computational complexity.

==> InputFiles/Introduction.tex <==
	\vspace{\sectionshift}
	\label{sec:intro}

% [Ready for feedback]
% The future generation wireless systems are expected to cater to numerous applications with demanding requirements, such as high-data rates, ultra-low latency, and increased robustness. In addition to communication, a key feature of 6G technologies will be integrated localization and sensing services that come with their own performance demands and implementation challenges. Depending on the use-case scenario, the goal is to reach centimeter-level positioning accuracy, and millisecond-level latency \cite{BehravanVTM2023}. 

% The concept of \glspl{lis} as a sub-category of \gls{dmimo} systems, has been proposed for both communication and positioning \cite{Hu_LTS_TSP2018} and the practical realization for communication algorithms with \gls{lis} studied\cite{SanchezICCW2020},\cite{SanchezTSP2022}, showing promising results of \gls{lis} being a key enabler for advancing the current wireless systems. However, in order to close the performance gaps between 5G and 6G, and achieve joint communication and positioning, there will be a need for low-latency and high-accuracy positioning algorithms compatible with the distributed communication infrastructure.


% \cite{WildingEUCNC2023}

6G is expected to feature advancements such as large signal bandwidth and array aperture, and a more decentralized network structure with \gls{dmimo} serving as key physical layer solution \cite{GustavssonJOM2021}. %,partially solving implementation problems  
Together, these features enhance integrated sensing capabilities, potentially enabling centimeter-level localization, millisecond-level latency and high data rates, across various scenarios \cite{BehravanVTM2023} including urban and indoors characterized by severe multipath propagation, \gls{olos} and highly-dynamic channel conditions. Designing localization algorithms that are both computationally efficient and reliable across diverse system configurations and harsh channel conditions is both critical and challenging.
%Leveraging \glspl{mpc} associated with distinct environmental features has shown promise in improving localization robustness and accuracy, but it is often complicated by the unknown and changing number of visible environmental features. 

%Multipath-based localization can be interpreted as a framework that jointly addresses feature visibility detection, mobile agent localization, and measurement-origin uncertainty through data association.

For decentralized networks, effective data fusion scheme across distributed units is also critical.
Collectively, all the aspects leads to a high-dimensional and highly non-linear inference problem.

%\Gls{bp}, that works by passing ``messages'' for performing inference, provides an efficient and scalable solution for \gls{mpc}-based localization, and has shown state-of-the-art performance in various experiments \cite{} . 
\Gls{bp} works by passing ``messages'' along the edges of a factor graph that represents the underlying statistical model of the inference problem and provides an efficient and scalable solution for \gls{mpc}-based localization, and has shown state-of-the-art performance in various experiments \cite{Erik_SLAM_TWC2019, XuhongICC2024, LeitingerICLGNSS2016} . % and typically uses the particle-based implementation.  
% \paragraph{State-of-the art}mention radio \gls{slam} and positioning algorithms. Mention that there is no latency and hardware analysis for these types of algorithms, implementability.
% \gls{mpc}-based methods that exploits multipath by estimating \glspl{mpc} and associating them to \glspl{va} representing the location of the mirror image of \glspl{pa} on reflective surfaces. The locations of \glspl{va} are assumed to be know a priori.
% motivation of choosing this approach, state-of-the-art performance proven by many works, FG, highly scalable...
% more reference about ohter D MIMO algorithms and why we choose the BP algorithm
 % State-of-the-art \gls{mpc}-based \gls{slam} and positioning algorithms present very good accuracy, and 


%Although efforts to lower the computational complexity are continuously being done \cite{ AlexTWC2024, Erik_SLAM_TWC2019}, \gls{mpc}-based algorithms still remain computationally intensive, due to \gls{pda} and their particle-filter based implementation. 

Run-time analyses for some of these algorithms have been conducted, providing rough initial estimates of the expected latency \cite{AlexTWC2024,  Erik_SLAM_TWC2019, Florian_Proceeding2018} that however exceed the latency limits for the expected 6G use-cases, such as collaborative robots \cite{BehravanVTM2023} ($1-10$\,ms) or XR-AR applications \cite{HazarikaSensors2023} ($1-5$\,ms). Ultimately, a fast and efficient localization solution, benefits from the co-design of algorithm, topology and hardware implementation as it was shown, for example, in the case of deep neural networks\cite{StuderJSAC2025}.

\begin{figure}[!t]
    \centering 
        \includesvg[width=0.95\columnwidth]{Figures/scenario1.svg}
      %  \vspace{\captionshift}
    \caption{Depiction of the indoor scenario with distributed panels, equipped with antenna arrays and local processing capabilities. The data-flow between panels with known positions $\V{p}_{\mathrm{pa}}^{(j)}$, follows a daisy-chain topology. At any time $n$, an unknown number of LoS paths, that can be obstructed by the middle walls, are visible to the agent with position $\V{p}_{n}$. \rd{legend, (1) add one for agent; (2) ground truth, change to true agent positions/track}
    %The \gls{los} paths can be obstructed by the middle walls.
    }
    \label{fig:pos}
\end{figure}

The main contributions of this work are as follows: (i) we introduce a \gls{bp} localization algorithm adaptable to panelized \gls{dmimo} topologies, that allows us to only use the \gls{los} paths, lowering the computational complexity. Unlike some centralized algorithms that may incur high latency due to centralized data aggregation and processing, the distributed algorithm performs local processing with minimal inter-panel communication. The unified operations processed at each panel, facilitate system scalability without the need for hardware redesign; (ii) we formulate a hardware-assisted latency model based on the \gls{fpga} implementation of the building processing blocks of the algorithm, allowing us to make system-level trade-offs and to achieve a more accurate estimate of the potential latency for a real deployment case. The model can serve as an aid for fast design-space exploration for future testbed implementations and it strengthens the theoretical assumptions by revealing the bottlenecks from a latency and hardware-resource perspective;
(iii) we apply the algorithm to a dynamic indoor scenario with \gls{olos} conditions and  show the trade-offs between different key design parameters, such as array size, number of panels and particle count together with latency, that can serve as input for further optimizing the algorithm and hardware implementation through algorithm-hardware co-design. 
Additionally, we use a \gls{mpc}-based algorithm as a performance benchmark and demonstrate that the simpler \gls{los}-based approach achieves comparable accuracy as the number of panels increases. This shows that the system can trade a higher panel count for reduced algorithmic processing complexity, without much latency overhead.


%------------------------------------------------------------------------
% \cblue{contribution, (1) no need centralized system, minimum data traffic between panels only. achieving good performance. (2) presenting trade-off of key design features, provide important insights to the future hardware system/algorithm design.}

%We show the trade-off between the complexity of algorithm and the level of distribution of the wireless system. Under specific conditions, the algorithm enables high localization accuracy while maintaining low complexity.

% \rd{emphasize the contribution from the perspective that, hardware implementation of a highly efficient and scalable state-of-the-art MPC-based localization algorithm, applied to an dynamic indoor scenario with OLOS conditions and considering measurement impairments, clutters...., providing important insights of hardware and algorithm co-design.....}

% To overcome some of the compute-intensive task challenges, we consider a \gls{los}-based distributed belief-propagation localization algorithm, co-designed with a \gls{dmimo} topology, compatible with communication tasks. We formulate a hardware-assisted latency model based on the \gls{fpga} implementation of the building processing blocks of the algorithm and compute the latency for different panel configurations and number of particles, to achieve a more accurate estimate of the potential latency for a real deployment case. The model can serve as an aid for fast design-space exploration for future testbed implementations. Moreover, it strengthens the theoretical assumptions by revealing the bottlenecks from a latency and hardware-resource perspective. 
% Furthermore, we take a \gls{mpc}-based algorithm as a performance benchmark that exploits multipath by estimating \glspl{mpc} and associating them to \glspl{va}, that represent the location of the mirror image of \glspl{pa} on reflective surfaces. We show that the simpler, \gls{los}-based algorithm has a similar performance in terms of accuracy with an increasing number of panels, thus being able to trade off a higher number of panels for a lower processing complexity of the algorithm. 

% \gls{mpc}-based methods that exploits multipath by estimating \glspl{mpc} and associating them to \glspl{va} representing the location of the mirror image of \glspl{pa} on reflective surfaces. The locations of \glspl{va} are assumed to be know a priori.


% Also mention the tradeoff of lower processing complexity with more panels
% We  develop a hardwrae assisted latency model and calculate the latency for a panelized LIS system for fast design space exploration



